Byzantine-Secure Relying Party for Resilient RPKI

To protect against prefix hijacks, Resource Public Key Infrastructure (RPKI) has been standardized. To enjoy the security guarantees of RPKI validation, networks need to install a new component, the relying party validator, which fetches and validates RPKI objects and provides them to border routers. However, recent work shows that relying parties experience failures when retrieving RPKI objects and are vulnerable to attacks, all of which can disable RPKI validation. Therefore even the few adopters are not necessarily secure. We make the first proposal that significantly improves the resilience and security of RPKI. We develop BRP, a Byzantine-Secure relying party implementation. In BRP the relying party nodes redundantly validate RPKI objects and reach a global consensus through voting. BRP provides an RPKI equivalent of public DNS, removing the need for networks to install, operate, and upgrade their own relying party instances while avoiding the need to trust operators of BRP nodes. We show through simulations and experiments that BRP, as an intermediate RPKI service, results in less load on RPKI publication points and a robust output despite RPKI repository failures, jitter, and attacks. We engineer BRP to be fully backward compatible and readily deployable - it does not require any changes to the border routers and the RPKI repositories. We demonstrate that BRP can protect many networks transparently, with either a decentralized or centralized deployment. BRP can be set up as a network of decentralized volunteer deployments, similarly to NTP and TOR, where different operators participate in the peering process with their node, and provide resilient and secure relying party validation to the Internet. BRP can also be hosted by a single operator as a centralized service, e.g., on one cloud or CDN, and provides RPKI validation benefits even when hosted on a single network.

==> overview.tex <==
\begin{new}
\section{Overview of RPKI}\label{sc:rpki}
The goal of RPKI is to provide an authenticated information on prefix ownership in the Internet, which the routers can use for making routing decisions in BGP. 

{\bf Signed authorizations.} RPKI associates public keys with IP prefixes~\cite{rfc6480}. At the root Regional Internet Registries (RIRs) delegate the right to generate Route Origin Authorizations (ROAs) to customer LIRs (Local Internet Registries) which own the respective IP blocks. ROAs authorize AS numbers to advertise those prefixes in BGP. 
ROAs are stored in repositories hosted on hierarchically organised publication points [RFC6481]. The publication points are operated either in a hosted mode, e.g., by the RIRs, or in a delegated mode by an owner AS.

 {\bf Validation with relying party software.} The validation is performed with the relying party implementations, which contain hardcoded Trust Anchor Locators (TALs) to the root certificates of the RIRs. The retrieval of the objects is performed over RRDP or rsync protocol. Both protocols for retrieval of RPKI objects are not secure and do not authenticate the objects. The security relies on X.509 and on manifests to ensure integrity and completeness of repository contents.
 
 {\bf Traversal of publication points.} A relying party fetches the RPKI objects periodically, during each refresh interval by traversing the tree of each of the five RIRs. The refresh interval is defined in the relying party implementations. During the validation a relying party contacts every TAL known to it and downloads RPKI objects from every publication point it finds. Relying parties have two types of data caches: \textit{rpki-cache} contains the files downloaded from publication points (ROAs, MFT, CRLs, etc) and \textit{ROA-cache} contains the validated ROAs. The rpki-cache is updated in real time as the download takes place, the ROA-cache is updated after the validation process has finished. 
 
 {\bf ROV filtering.} The border routers query the ROA-cache periodically over the RTR protocol [RFC8210]. The routers trust the caches and use the cached objects for enforcing ROV. Border routers should reject BGP announcements which conflict with the ROAs, but accept announcements for which no ROAs could be fetched.

{\bf Interaction between components in RPKI.} We show the components and the interaction between them in networks that deployed RPKI and perform ROV in Figure~\ref{fig:rpki_process}. In step (1) a relying party software uses a DNS resolver to lookup the address of hardcoded TALs to locate the publication points of all 5 RIRs. The DNS resolver sends a lookup request to the nameserver (in the example in Figure \ref{fig:rpki_process} the nameserver is in the domain of the RIPE NCC RIR) to fetch the publication point's IP address (Step 2). In Step (3), the relying party connects to the publication point via RRDP or RSYNC to fetch the RPKI objects (ROAs, resource certificates, manifests, CRLs,...). The certificates may also delegate the responsibility for generating ROAs to another CA. In our example, the LIR \textit{example.com} uses the \textit{delegated RPKI} in which case the RIR's publication point only contains a certificate which delegates responsibility to the LIRs CA and contains the hostname of the LIRs publication point. Consequently, to download the actual ROAs, the relying party has to lookup the IP address of the LIR's publication point (Step 4) which leads the local DNS resolver to connect to the corresponding nameserver to fetch the IP address (Step 5). The relying party can then connect to the LIR's publication point and download the ROAs (Step 6). Finally the relying party compiles a list of IP prefixes and ASes which are allowed to announce those IP subnets. The border routers retrieve that list from the ROA-cache via the RTR protocol (Step 7). That list contains all RPKI data for any network in the world. BGP routers use the RPKI data to perform ROV: validate announcements they receive from other networks (Step x). If any of the Steps 1-6 fail, e.g., because of a benign failure or malicious attack, relying parties fall back to cached ROAs, fetched in the last update cycle, as long as these are available and not stale. Consequently, any attack on the availability of the connections done in steps (1-6) might lead to failure in retrieving ROAs from the RPKI tree and therefore can change the behaviour of the victim network when accepting BGP announcements.
\end{new}



\begin{figure}
    \centering    
    \includegraphics[width=0.45\textwidth]{res/rpki1-crop.pdf}
    \caption{RPKI process with RIPE NCC Regional Internet Registry (RIR) and
    {\it example.com} Local Internet Registry (LIR).}
    \label{fig:rpki_process}
\end{figure}



